"What is the value of {templates}?" Rethinking Document Information Extraction Datasets for LLMs

The rise of large language models (LLMs) for visually rich document understanding (VRDU) has kindled a need for prompt-response, document-based datasets. As annotating new datasets from scratch is labor-intensive, the existing literature has generated prompt-response datasets from available resources using simple templates. For the case of key information extraction (KIE), one of the most common VRDU tasks, past work has typically employed the template "What is the value for the {key}?". However, given the variety of questions encountered in the wild, simple and uniform templates are insufficient for creating robust models in research and industrial contexts. In this work, we present K2Q, a diverse collection of five datasets converted from KIE to a prompt-response format using a plethora of bespoke templates. The questions in K2Q can span multiple entities and be extractive or boolean. We empirically compare the performance of seven baseline generative models on K2Q with zero-shot prompting. We further compare three of these models when training on K2Q versus training on simpler templates to motivate the need of our work. We find that creating diverse and intricate KIE questions enhances the performance and robustness of VRDU models. We hope this work encourages future studies on data quality for generative model training.

==> appendices/a0pastdatasets.tex <==
% Not sure if this is needed in the appendix or main paper

\section{Past datasets and drawbacks}
\begin{itemize}
    \item FLAN \citep{wei-22-finetuned}: Dataset for general NLP tasks. Each task/dataset gets 10 templates to fill for diversity. Furthermore, each task/dataset has up to three additional templates that ask for generation. No task regarding information extraction so no direct comparison to how questions exactly from the text are given (closest is reading comprehension).
    \item Flan-PALM \citep{chung-22-scaling}: Similar to FLAN but encorporates additional datasets
    \item InstructGPT \citep{ouyang-22-training}: Not really relevant, did not convert any datasets
    \item Self-Instruct \citep{wang-23-self}: Again not really converting datasets
    \item LlamaV2 \citep{touvron-23-llama}: Used dialogue datasets
    \item mPlug-DocOwl \citep{ye-23-mplug}: DocAI Dataset. For Information extract, questions are created used a single template with no alternatives. Very not diverse
    \item UDOP \citep{tang-23-unifying}: Like mPlug-DocOwl, only uses one  template
    \item DUDE benchmark \citep{landeghem-23-document}: General new VQA dataset
    \item 
\end{itemize}

\section{Other Relevant Work}
\begin{itemize}
    \item \citet{hegde-23-analyzing}
\end{itemize}

==> deprecated/2related.tex <==
\section{Related Work}\label{sec:related}
\begin{comment}
    Describe the broader context of VRDU literature in which this work sits which this data set ultimately hopes to enrich
\end{comment}

% With the rise of LLMs and foundational generative models that treat information extraction and classification tasks through unstructured prediction (i.e., generation), the field of VRDU has had to adapt its datasets and tasks away from structured and span-based outputs.
% In this section, we describe the VRDU dataset and modeling literature before addressing the gaps that this paper targets in \cref{sec:kie}.

\begin{comment}
    Describe some classical KIE data sets and tasks. Mention all relevant datsets, but spend longer on the datasets we transform.
\end{comment}

% \subsection{General Overview of VRDU}

\paragraph{Datasets.} VRDU spans a multitude of tasks, including document classification \citep{harley2015icdar}, document structure prediction \citep{jaume2019funsd, vu-2020-revising, li2020docbank, xu-etal-2022-xfund, zmigrod-2024-treeform}, and visual question answering (VQA) \citep{mathew2021docvqa, landeghem-23-document}.
In this work, we focus on KIE due to the abundance of existing datasets as well as its importance in enterprise applications.
Several KIE datasets cover invoice and receipt documents \citep{huang-2019-icdar, park2019cord, sun-2021-spatial, simsa2023docile};
these are particularly interesting due to \defn{line items}, which are connected entities such as an item's name and price.
Other KIE datasets also examine document types such as forms or legal documents \citep{jaume2019funsd, Borchmann2021DUEED, stanislawek-2021-kleister, wang-2023-vrdu, zmigrod-2024-buddie}.
% Many KIE datasets such as CORD \citep{park2019cord}, Docile \citep{simsa2023docile}, SROIE \citep{huang-2019-icdar}, and WildReceipt \citep{sun-2021-spatial} cover invoice and receipt documents.
% CORD and Docile are particularly interesting due to the presence of \defn{line items}, which are rows of connected entities that are useful to test a model's ability to understand entity interactions.
% Line items may be used to test if a model can understand the localization of entities and how they interact with other entities.
% KIE Datasets such as BuDDIE \citep{zmigrod-2024-buddie}, DeepForm \cite{Borchmann2021DUEED}, Kleister Charity (KLC) and NDA \cite{stanislawek-2021-kleister}, VRDU Ad-Buy (Ad-Buy) and Registration Form (Reg. Form) \cite{wang-2023-vrdu}\footnote{VRDU Ad-Buy is a subset of DeepForm, but contains a richer annotation scheme.} consider other document domains such as forms and reports.\footnote{While FUNSD \citep{jaume2019funsd} is often considered a KIE dataset, its entities are structural components such as header, question, and answer. We thus consider it to be more in line with document structure prediction tasks.}
\cref{tab:kie-datasets} provides details on available KIE datasets.\footnote{We only focus on English datasets in this work. Nevertheless, other non-English VRDU datasets exist \citep{wang-2021-towards, qi-2022-dureadervis, ding-2023-form}.}
% Note that the aforementioned datasets are all in English; non-English KIE datasets also exist \cite{qi-2022-dureadervis}, though we do not cover any in this work.

\input{tables/kie_datasets}

\begin{comment}
    Describe some classical methods used for document understanding like Layout LM and methods that predate it.
\end{comment}

\paragraph{Models.}
There are two primary modeling paradigms in VRDU: OCR-based models and OCR-free models.
OCR-based models \citep{xu2020layoutlm, peng-2022-ernie}), rely on a combination of text, spatial (bounding box information), and often vision features.
% The text and spatial features are extracted using OCR tools while the vision features are extracted from the document image.
Alternatively, OCR-free models \citep{davis-2022-end, kim-2022-ocr, lee-2023-pix2struct}, Donut \citep{kim-2022-ocr}.
As one may expect, OCR-based models tend to outperform OCR-free models \citep{tang-23-unifying}; however, they require expensive OCR engines to be used as a pre-processing step.
% this comes at a cost as OCR engines can be computationally expensive and error-prone.
Multi-modal LLMs have recently been proposed to tackle VRDU tasks, utilizing both OCR-based \citep{wang2023docllm, tanaka-2024-instructdoc} and OCR-free \citep{ye-2023-ureader, ye-23-mplug, hu-2024-docowl} models.
% Some have adopted OCR-based approaches, such as DocLLM \citep{wang2023docllm} and InstructDr \cite{tanaka-2024-instructdoc}, while others have preferred OCR-free approaches, such as UReader \citep{ye-2023-ureader} and mPLUG-DocOwl \citep{ye-23-mplug, hu-2024-docowl}.


==> deprecated/3kie.tex <==
\input{figures/example_questions}

\section{Key Information Extraction with LLMs}\label{sec:kie}
% \Mathieu{Do we have a 2.2 subsection too?
% \response{Ran} No but it still falls under related work but is too big for a paragraph. It's ok to have a single subsection :)
% }

\begin{comment}
    Discuss the use of LLMs in VRDU

    Discuss instruction tuning/prompt tuning and how that is used in LLMs. Such data sets are similarly needed for VRDU 

    Overview of the three main approaches for creating datasets for LLMs (including advantages and disadvantages:
        1. Using simple templates
        2. Getting human annotators to create data
        3. Getting LLMs to generate data

    Our method is somewhere between 1 and 2, can hint at this but don't go into details yet.
    
    Benchmarks to describe and briefly distinguish from our work: DUE, DUDE, InstrucDoc
    
    Describe QA data sets released as part of UReader and any other similar papers. 
\end{comment}

Generative LLMs are both trained and evaluated by using a prompt that gives the model a task and a response that the model has to generate.
To utilize LLMs for traditional information extraction tasks, said tasks must be formulated into a prompt-response type structure.
% In this paper, we consider this transformation for key information extraction, the most popular VRDU task in terms of associated datasets.
So far, the VRDU and NLP literature has proposed three main strategies to obtain such formulations: populating simple templates based on existing annotations, manually curating questions, or generating questions using LLMs.
We discuss the advantages and disadvantages of each method below to motivate our approach in \cref{sec:dataset}.

\paragraph{Populating Simple Templates.}
The most common method for designing large datasets of instructions for LLMs is templating.
This is the case in both general NLP \cite{chung-22-scaling, wei-22-finetuned} as well as in VRDU \cite{tang-23-unifying, ye-2023-ureader, zhang-2023-llavar, wang-2023-vrdu, tanaka-2024-instructdoc, zmigrod-2024-buddie}.
Templating is a cost-effective technique for generating prompt-response pairs based on annotations since only a handful of templates may be needed to cover a task.
Unfortunately, most templating approaches in VRDU rely on simplistic and dataset-agnostic templates that do not reflect a model's true understanding of the task nor the real-life queries that would be submitted to a generative model.
For instance, several works use a single template for the KIE task, which asks, ``What is the value for the \texttt{\{key\}}?'' \citep{ye-2023-ureader, ye-23-mplug, wang2023docllm, hu-2024-docowl}, often leading to under-specified questions when many values for the same key are present in a document.

\paragraph{Manually Constructing Questions.}
Rather than relying on existing datasets, researchers can
% use annotation tools and annotators to
construct prompt-response datasets from the ground up such as DocVQA \citep{mathew2021docvqa, tito-2022-hierarchical} and DUDE \citep{landeghem-23-document}.
The literature has previously used VQA datasets from similar domains due to the lack of in-domain datasets
% to bolster the amount of data available for training and evaluation 
\citep{Borchmann2021DUEED, mathew-2022-info, tanaka-2024-instructdoc}.
The benefits of human-annotated datasets come from the quality, diversity, and in-depth questions that can be achieved.
Unfortunately, curating VQA datasets is expensive, and thus, creating datasets of the scale needed to instruction-tune LLMs can be inaccessible to many practitioners.

\paragraph{Generating Questions using LLMs.}
Past work has demonstrated that utilizing LLMs to create fine-tuning datasets may be a promising research avenue
\citep{honovich-2023-unnatural, peng-2023-instruction, cheung-etal-2024, alpaca, wang-23-self}.
% demonstrated that utilizing LLMs to create fine-tuning datasets may be a promising research avenue.
% Similar results were given in \citet{honovich-2023-unnatural}, \citet{alpaca}, and \citet{wang-23-self}.
This also includes work for multi-modal vision LLMs \citep{haotian-2023-visual, li-2023-blip}, suggesting this methodology can extend to VRDU.
To our knowledge, however, the VRDU literature has not used LLMs to generate prompt-response pairs.
Such work must be mindful of the potential shortcomings of this approach \citep{gudibande-2023-false}.

% The work presented in the remainder paper is a collection of KIE datasets that have been transformed into prompt-response type datasets.
The methodology followed in this paper lies between populating templates and manually curating questions. 
We design a broad set of intricate templates for each KIE dataset, optimizing for quality and diversity of question types.
We believe that leveraging LLMs to bolster the variety of our templates could lead to promising and exciting future work, though we do not explore this further.

% As a future direction we could prompt LLMs to generate more templates/reformulations of our templates in a few shot setting

==> tables/instruction_tuning.tex <==
\begin{table}[]
    \centering
    \small
    \begin{tabular}{l rrr}
         \bf Model & \bf \simpleDatasetName & \bf \sampledDatasetName & \bf \datasetName \\
         \midrule
         Donut \\
         Pix2Struct \\
         DocLLM \\
    \end{tabular}
    \caption{ANLS scores on DUDE test set using instruction tuning on \simpleDatasetName, \sampledDatasetName, and \datasetName.}
    \label{tab:instruction-tune}
\end{table}
